"We Need Structured Output": Towards User-centered Constraints on Large Language Model Output

Large language models can produce creative and diverse responses. However, to integrate them into current developer workflows, it is essential to constrain their outputs to follow specific formats or standards. In this work, we surveyed 51 experienced industry professionals to understand the range of scenarios and motivations driving the need for output constraints from a user-centered perspective. We identified 134 concrete use cases for constraints at two levels: low-level, which ensures the output adhere to a structured format and an appropriate length, and high-level, which requires the output to follow semantic and stylistic guidelines without hallucination. Critically, applying output constraints could not only streamline the currently repetitive process of developing, testing, and integrating LLM prompts for developers, but also enhance the user experience of LLM-powered features and applications. We conclude with a discussion on user preferences and needs towards articulating intended constraints for LLMs, alongside an initial design for a constraint prototyping tool.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> sections/old_sections/sec-010-intro-20240105.tex <==
\section{Introduction}

Over the past few years, we have witnessed the extraordinary capability of Large Language Models (LLMs) to generate responses that are not only creative and diverse but also highly adaptable to various user needs \cite{ouyang_training_2022,brown_language_2020,chowdhery_palm_2022,petridis_promptinfuser_2023,liu_what_2023}. 
This accessibility has empowered scientists, developers, entrepreneurs, and enthusiasts to easily and rapidly prototype and build AI functionalities \cite{jiang_promptmaker_2022,jiang_genline_2021,petridis_constitutionmaker_2023,park_generative_2023,liu_selenite_2023} without extensive requirements in machine learning (ML) or natural language processing (NLP) expertise \cite{wu_promptchainer_2022,wu_ai_2022,terry_ai_2023,jiang_promptmaker_2022}. 
For example, researchers can prompt ChatGPT \cite{openai_chatgpt_2023} to condense long articles into concise summaries for fast digestion; while video game developers can generate  detailed character profiles with rich personality traits, backstories, and unique abilities on demand, simply by dynamically prompting an LLM with the game context and players' preferences. % can cut these examples if they are not essential


As much as end-users appreciate the unbounded creativity of LLMs, recent field studies examining the development of LLM-powered applications have repeatedly demonstrated the necessity to \emph{impose certain constraints} on LLM \cite{parnin_building_2023,petridis_promptinfuser_2023,fan_large_2023}. For instance, a user might require a summary of an article to be ``strictly less than a 20 words'' to meet length constraints, or a generated video game character profile to be ``valid JSON that can be parsed by Python'' to be integrated into a development pipeline.
However, as evidenced by many recent NLP benchmarks and evaluations \cite{sun_evaluating_2023,zhou_instruction-following_2023,zeng_evaluating_2023}, current state-of-the-art LLMs still lack the ability to \emph{guarantee} that the generated output will conform to user-defined constraints in the prompt (sometimes referred to as \emph{controllability}). Although researchers have proposed various methods to improve \textit{controllability}, such as supervised fine-tuning with specialized datasets \cite{sun_aesop_2021} or controlled decoding strategies \cite{xu_look-back_2023,beurer-kellner_prompting_2023,mudgal_controlled_2023,noauthor_guidance-aiguidance_2023}, they tend to only focus on addressing a narrow range of constraints without taking into consideration the diverse usage scenarios and rationale that real-world developers and end-users encounter when prototyping and building practical LLM-powered functionalities and applications \cite{lu_neurologic_2022,hokamp_lexically_2017,hu_improved_2019}.


In this work, we take the first step to systematically investigate the scenarios and motivations for applying output constraints from a \emph{user-centered perspective}. Specifically, we sought to understand: 

\begin{itemize}
    \item RQ1: What are the different types of real-world use cases that necessitate or could benefit from being able to constrain LLM outputs?
    
    \item RQ2: What are the benefits and impacts of being able to apply constraints to LLM outputs?
    % The importance of having constrained output and subsequent impact on their workflows;
    
    \item RQ3: How would users like to articulate their intended constraints to LLMs?
\end{itemize}

We investigated these research questions by developing a survey to a broad population of industry professionals (software engineers, researchers, designers, program managers, etc.) who have experience with prompt-based prototyping \cite{jiang_promptmaker_2022} and building LLM-powered applications. 
Our analysis identified six primary categories of output constraints that users desire, each supported by detailed usage scenarios and illustrative examples (Table \ref{tab:use-case}). In a nutshell, users not only need low-level constraints, which mandate the output to conform to a structured format (for example, valid JSON or a specific custom template) and an appropriate length, but also desire high-level constraints. These high-level constraints involve  semantic and stylistic guidelines that users would like the model output to adhere to without deviation from reality or users' original intent. Notably, developers reported having to write ad-hoc yet complicated parsing and plumbing logic in order to defend against ill-formed LLM output, which can be significantly simplified, or even eliminated entirely, should LLMs can guarantee that the generated output adheres to predefined constraints. The ability to apply constraints could also streamline the integration with existing product pipelines, help satisfy UI requirements and product restrictions, as well as improve overall user experience and trust towards LLM-powered features and applications.


Finally, we \temp{how to express controls}


Overall, this paper contributes:

\begin{itemize}[leftmargin=.2in]
% \setlength\itemsep{-0.2em} 
    \item \temp{Findings from a survey of 63 respondents, contributing a broad set of use cases ...}
    
\end{itemize}



% \temp{Based on the survey, we further created a GUI + controlling mechanism to exercise control, bridging the gap.}


% Recent work in ML and NLP has proposed various methods to improve the \textit{controllability} of language models, such as supervised finetuning with carefully-curated datasets \needcite or constrained decoding strategies \needcite. In the meantime, researchers have handcrafted various benchmarks to evaluate said controllability, such as Numerical Planning Benchmark \cite{sun_evaluating_2023} and IFEval \cite{zhou_instruction-following_2023}. 


% \temp{
% to combat, few shot (not coverage), and (see hci research proposal) --- a gap between user's intent for control and the ability for the model to interpret and follow those controls during generation.
% }


% \temp{
% a lack of understanding of what possible constraints that end-users want, how would that impact their workflows, and how they prefer to express those constraints.
% }

==> sections/old_sections/sec-020-methods-20240105.tex <==
\section{Methods: Survey}\label{sec:methods}

To get a broad range of insights from people who have experience with prompting and building LLM-powered applications, we deployed an online survey to users of an internal prompt-based prototyping platform (similar to the OpenAI API Playground \cite{openai_playground_2023} and Google AI studio \cite{google_google_2023}) at a large technology company. We chose this platform because it was explicitly designed to lower the barriers to entry into LLM prompting and encourage a broader population (beyond machine learning professionals) to prototype and develop LLM-powered applications. 
We publicized the survey through the platform's user mailing list. Participants was rewarded \$10 USD for their participation. We ran the survey for two weeks during Fall 2023. Participants were required to be at least 18 years old and fluent in English.

\subsection{The Survey Instrument}
Our survey started with questions concerning participants' background and technical proficiency, such as their job roles, their level of experience in designing and engineering LLM prompts, and the ways in which these prompts are utilized. 
The survey subsequently investigated RQ1 and RQ2 by asking participants to report \emph{three real-world use cases} in which they believe the implementation of constraints to LLM outputs is necessary or advantageous. For each use case, they were encouraged to detail the specific scenario where they would like to apply constraints, the type of constraint that they would prefer to implement, the degree of precision required in adhering to the constraint, and the importance of this constraint to their workflow.

Finally, the survey investigates RQ3 by asking participants to reflect on scenarios where they would prefer \emph{expressing constraints via GUI} (sliders, buttons, etc.) over natural language (in prompts, etc.) and vice versa, as well as any alternative ways they would prefer to articulate constraints to LLMs. 

% \temp{some justification on why we chose ``GUI'' as an alternative to ``natural language''
% - need for prototyping
% - mimicking temperature, top-p controls, stop word, etc.}
% \temp{consider framing this as a case study}

% \temp{
% The survey then asked participants to reflect through open response on scenarios where they would prefer \emph{expressing constraints via GUI} (sliders, buttons, etc.) over natural language (in prompts, etc.) and vice versa, as well as any alternative ways they would prefer to express constraints. 
% To facilitate the reflection, the survey additionally asked participants to rate their level of preference in: 
% 1) control output length (e.g. exactly 3 words, no more than 3 paragraphs, etc.); 2) constrain output to a predetermined set of options (e.g. only output ``left-handed'', ``right-handed'', or ``ambidextrous''); 3) output in a specific format/structure (e.g., bulleted/ordered list, JSON, custom template); 4) literal matching (must include or avoid certain words/phrases); 5) semantic constraints (e.g. must cover or avoid certain topics, only use certain libraries when generating code); 6) stylistic constraints (e.g. mimicking Yoda/Shakespeare/certain personas).
% Each question presented a 7-point Likert scale from ``strongly prefer natural language'' to ``strongly prefer GUI.''
% }


Detailed survey questions are documented in section \ref{sec:apx-survey-instrument} of the Appendix.


\subsection{Data Analysis}

We received 51 individual survey responses, adding up to \temp{143} unique use cases. To analyze the contents of the open-ended responses, the first author first read through all responses. They then used an inductive analysis approach \cite{strauss_basics_1990} to generate and refine themes for each research question with frequent discussions with the research team. We present the resulting themes for each research question starting in section \temp{x}.  



\subsection{Study Design Limitations}

The survey was primarily focused on industry professionals experienced in prompting and building LLMs. Consequently, our respondents may not represent the entire spectrum of LLM users. That said, we postulate that industry professionals, including software engineers and UX designers, may express a much stronger desire for output constraints on LLMs, which would facilitate the integration of LLMs into existing systems and workflows. Output constraint might likely to be of lesser concern for non-professional or amateur users who interact with LLMs more casually, e.g., through chat interfaces. The exploration of this particular user group, however, is beyond the scope of our current study.

In addition, compared to other large-scale surveys \cite{cai_software_2019}, we only garnered a relatively small number of individual responses, which might limit the statistical power and generalizability of the findings.
A potential obstacle could be attributed to our survey design --- we largely relied on open-ended questions, which, while helpful for capturing a variety of perspectives, placed a heavy cognitive and physical load on the respondents to fill out.
However, one encouraging observation was that towards the end of the deployment, the influx of novel and unique findings began to taper off, suggesting we had reached a point of saturation and thus a reasonable stopping point for our survey.






==> sections/old_sections/sec-030-demographics.tex <==
% \section{Job Roles and Prior Experience with LLMs}

% To understand the context of our respondents' perspectives, we first describe their job roles and levels of experiences with prompting LLMs. 
To begin, over half of our respondents were software engineers (58.8\%) across various product teams; others held a variety of roles like consultant \& specialist (9.8\%), analyst (7.8\%), researcher (5.9\%), UX engineer (5.9\%), designer (3.9\%), data scientist (3.9\%), product manager (2.0\%), and customer relationship manager (2.0\%).
All respondents had experience with prompt design and engineering, with the majority reported having extensive experience (62.7\%).
The targeted audience and use cases of their prompts were split approximately evenly among consumers and end-users (33.3\%), downstream development teams (31.4\%), or both (29.4\%), with some created specifically for exploratory research \& analysis (5.9\%).\looseness=-1


==> sections/old_sections/sec-031-use-cases-20240105.tex <==
\section{Real-world Use Cases that Necessitate Output Constraints}\label{sec:use-cases}

\input{use-cases-table}

Table \ref{tab:use-case} shows six main categories of use cases that necessitate output constraints, which can be further divided into low-level versus high-level constraints. We now discuss these categories in detail with representative examples.

\subsection{Low-level Constraints}

\subsubsection{Structured Output}\label{sec:use-case-structured-output}
By far the most frequently mentioned use case for constraints is to specify the structure of the output (\temp{xx\%}). A substantial portion of respondents mentioned that, similar to traditional API calls, they would like LLM outputs to also be valid JSON objects that can be seamlessly \userquote{parsed and integrated into downstream applications.} Notably, OpenAI has recently rolled out a ``JSON mode'' API for GPT-series models that constrains a model to only generate strings that parse into valid JSON object \cite{openai_json_2023}, however, our survey respondents thought this was not sufficient, and hope to have finer control over the schema of the JSON: \userquote{I expect the quiz [that the LLM makes given a few passages provided below] to have 1 correct answer and 3 incorrect ones. I want to have the output to be like a json with keys \texttt{\{"question": "...", "correct\_answer": "...", "incorrect\_answers": [...]\}}.}
In addition, respondents mentioned the need for various other types of structures, including standardized formats like \userquote{markdowns} or \userquote{HTML} as well as custom templates like \userquote{bulleted list} or even \userquote{DSL (domain specific language) [for enterprises].} It's important to note that some respondents reported that \userquote{few-shot prompts} (where the output format is demonstrated with a handful of examples) tend to work \userquote{fairly well} in terms of defining the output format. Nevertheless, they agreed that having a formal guarantee would certainly be appreciated (see section \ref{sec:importance-increase-prompt-dev-efficiency} for their detailed rationales).



\subsubsection{Multiple Choice}\label{sec:use-case-multiple-choice}
Another common use case that respondents reported is asking LLMs to select from a predefined list of options as the output (\temp{xx\%}). This could range from using LLMs for common classification and data labeling tasks such as \userquote{classifying student answers as right / wrong / uncertain} or \userquote{[classifying sentiments as] Positive, Negative, Neutral, Strongly Positive, etc.} to translating high-level user intent (e.g., \userquote{find my recent emails}) to supported API parameter(s) (e.g., \userquote{from / to / after / before}). It is worth noting that, in this particular use case,  respondents typically expect the model to output only the ``selection'', without trailing it with an ``explanation,'' as the addition of explanation could potentially confuse the downstream parsing logic.



\subsubsection{Length Constraints}\label{sec:use-case-length}
Respondents also emphasized the importance of being able to constrain the length of LLM outputs (\temp{xx\%}), such as \userquote{present[ing] [...] each major reason as a separate tweet under 280 characters} or \userquote{number of bullets [in a list]}. Contrary to structured output or multiple choice, respondents believed that it is impractical for the current generation of LLMs to strictly adhere to length constraints. Instead, they suggested that an approximate match is generally sufficient, for example, \userquote{110 words is ok as long as it is not a big blurb of 300 words or ore.} 



\subsection{High-level Constraints}

\subsubsection{Semantic Constraints}\label{sec:use-case-semantic}
Our survey revealed that respondents were interested in applying various types of semantic output constraints (\temp{xx\%}). Firstly, there is a desire for the ability to have the model exclude specific terms or items from the output (e.g., \userquote{excluding PII (personally identifiable information)}) or even \userquote{explicitly NOT do some particular task} (e.g., \userquote{DO NOT greet the user}). 
Conversely, respondents would also like to have the ability to make sure that the model must include certain information (e.g., must expressing gratitude in an email to manager). A special case here is for LLMs to recite a segment of the input in its output, sometimes with additional modifications: \userquote{We want LLM to repeat input with some control tokens to indicate the mentions. e.g. input: `Obama was born in 1961.',... , we want output to be `<<Obama>> was born in 1961.'} 
Thirdly, respondents indicated a preference for constraining LLMs to generate content that are centered around a certain topic or domain, ensuring relevance and coherence. To illustrate, one respondent desired that the output should consistently remain \userquote{in the same ballpark} as \userquote{the user's original query,} for example, \userquote{[the output of] a query about `fall jackets' should be confined to clothing.}
Last but not least, respondents wished for LLM-generated code to adhere to specific syntax, grammatical rules, or dialects and to utilize only the variables and methods defined within the given context. This would ensure that the code compiles and runs smoothly. For instance, one respondent to highlighted the importance to \userquote{restrict the output to a particular dialect (MySQL) and use the table / database name mentioned in the prompt} when generating SQL code.



\subsubsection{Stylistic Constraints}\label{sec:use-case-stylistic}
\temp{xx\%} of the use cases focused on constraining the tone and style of the output, such as \userquote{preference for active voice over passive voice} when summarizing news articles or using \userquote{straightforward language and avoid complex technical jargon} when explaining concepts to \userquote{someone with no technical background.}



\subsubsection{Preventing Hallucination}\label{sec:use-case-preventing-hallucination}
Last but not least, a non-trivial portion of the use cases focused on preventing LLM hallucination (\temp{xx\%}). On the one hand, respondents emphasized the necessity of ensuring that the LLM output stays grounded in the provided context and always be truthful, such as \userquote{include [...] only the real facts} and avoid hallucinating \userquote{opinions or beliefs} or \userquote{details or events that are not explicitly mentioned in the provided data} when summarizing documents or meeting notes. 
On the other hand, respondents expressed dissatisfaction with the current generations of LLMs, citing their tendency to ``improvise'' actions beyond the initial set of instructions.
For instance, one respondent recounted an experience where they asked an LLM to \userquote{annotate a method with debug statement.} Their expectation was for the output to \userquote{ONLY include changes that add print statements to the method,} however, they found that the LLM frequently introduced \userquote{changes in syntax} that were unwarranted. In such scenarios, respondents expressed a preference for constraining the LLMs to perform solely the requested actions, without any improvisation. We delve into the advantages of being able to constrain models from hallucinations in section \ref{sec:importance-ux}.



% \subsection{Others}\label{sec:use-case-others}



==> sections/old_sections/sec-032-importance-20240105.tex <==
\section{Benefits of Output Constraints}\label{sec:importance}





In addition to use cases of applying output constraints, our survey revealed a variety of potential impacts of applying output constraints that respondents believe might shift the status quo. These include both \emph{developer-facing} benefits, such as increasing prompt-based development efficiency (\temp{xx\%}) and streamlining integration with downstream processes and workflows (\temp{xx\%}), as well as \emph{user-facing} benefits, such as satisfying product and UI requirements (\temp{xx\%}) and improving user experience and trust of LLMs (\temp{xx\%}). Here are the most salient responses:


\input{importance-table}


\subsection{Increasing Prompt-based Development Efficiency}\label{sec:importance-increase-prompt-dev-efficiency}
The most prominently reported impact of being able to constrain LLM outputs is that it would increase the efficiency of prompt-based engineering and development (\temp{xx\%}), which stems from the workarounds that developers currently employ to overcome the inherent unpredictability of LLM outputs. Some specifically mentioned that their current process of crafting a prompt involves \userquote{spending time in defining the [output] format} that requires multiple iterations of trial and error (similar to what previous research has found \cite{zamfirescu-pereira_why_2023,parnin_building_2023}): \userquote{Currently, I have to evaluate with a dataset the impact of each prompt variation on the output to choose the best one.} Thus, having the ability to deterministically constrain the output format would speed up the process of prompt design and engineering, sometimes by \userquote{dozens of hours of work per week.}\looseness=-1

Another commonly reported practice is building custom yet complex infrastructure to parse, verify, and transform LLM generations into the desired format, sometimes referred to by respondents (mostly software engineers) as \userquote{massaging [the output] after receiving}. For example, developers oftentimes had to \userquote{chase down `free radicals' when writing error handling functions in JavaScript,} and felt necessary to include \userquote{custom logic to match and filter values} and \userquote{further verification/critic models in the pipeline.} Therefore, specifying constraints prior to generation may be the key to reduce the ad-hoc plumbing logic currently required post-generation, enhancing its maintainability (\userquote{[it would] make the response parsing code much simpler and easier to maintain}), and improve the overall developer experience (\userquote{it's a much nicer experience if these things (formatting the output in bullets) `just work' without having to implement additional infra...}).\looseness=-1

In addition, respondents envisioned that being able to guarantee that the output conform to a specific format would eliminate the necessity of having to \userquote{request multiple responses} from a model and \userquote{iterate through them until I find a valid response,} thereby saving inference costs and decreasing latency in the entire pipeline.





\subsection{Streamlining Integration with Downstream Processes and Workflows}\label{sec:importance-streamline-integration-with-downstream}

When considering LLMs as components within broader research and production pipelines, respondents recognized that the ability to constrain their output can effectively streamline their integration with downstream processes and workflows (\temp{xx\%}). In particular, when using LLMs to generate code, respondents stressed for the importance of constraints that would ensure that the generated code can successfully execute (e.g., \userquote{[the code] needs to be valid syntax and only call the methods specified in the context}), and avoid situations such as \userquote{[hallucinating] unsupported operators [that would] cause the API call to fail and fetch 0 results} or \userquote{if it generates SQL with a different table name and with different dialect, the SQL will not be execution worthy.} Note that recent ``function calling'' features introduced by OpenAI's GPT-series models \cite{openai_function_2023} as well as Google's Gemini-family models \cite{google_cloud_function_2023} partially address this concern by having an LLM ``select'' the appropriate function(s) to call from a predefined list of function descriptions, however, it leaves the responsibility of correctly \emph{implementing} a function to the user as opposed to the LLM itself.

Numerous previous studies have reported that LLM is an effective tool for generating synthetic datasets used in further AI training \cite{josifoski_exploiting_2023,eldan_tinystories_2023,viswanathan_prompt2model_2023}, and our survey respondents postulated that the ability to impose constraints on the model could significantly enhance the quality and integrity of these synthetic datasets. For example, \userquote{I want the model to not say a movie's name when it describes its plot. This is essential and a hard constraint, as I'm going to be training using this data for something that shouldn't know the movie's name (say a predictive model of the movie itself).} And, violations of constraints could \userquote{make the data point unusable.}

Furthermore, given the overarching industry trend of transitioning to newer or more cost-effective models as they become available \needcite, respondents emphasized the necessity of being able to \userquote{canonize} the constraints between models, as it would prevent the need for additional prompt-engineering post-migration: \userquote{if I switch model, I get the formatting immediately.} This suggests that instead of combining task instructions and constraints in the same prompt, it could be more advantageous, under certain circumstances, for users to provide output constraints as a parallel input to the model along with the prompt. Ideally, the prompt should now solely contain task instructions.



\subsection{Satisfying UI and Product Requirements}\label{sec:importance-satisfying-ui}

Respondents suggested that the ability to constrain the output is essential for meeting established user interface (UI) and product requirements (\temp{xx\%}), particularly when the output from LLMs will be displayed, directly or indirectly, to end users. One scenario involves incorporating LLM-generateed content into UI components that are of a specific size, necessitating stringent length constraints: \userquote{we are trying to display a teaser to a user: In these scenarios, the text from the LLM will be displayed directly to the user in an UI that cannot exceed certain bounds. Failure to meet these bounds usually means we have to throw away all the data because we can't fit it within the UI.} This issue is likely to become more pronounced on mobile devices, which have limited screen real estate \cite{liu_wigglite_2022}. The consistency of output length and format is also essential when it comes to user-facing content, and respondents emphasized that \userquote{too much variability in the generated text can be overwhelming to the user and clutter the UI.} Moreover, with the help of constraints, LLM-generated content can more effectively comply with character limits set by certain products or platforms, such as \userquote{a tweet under 280 characters} or a valid YouTube Shorts title that \userquote{stays under 100 characters.}


% \temp{cite promptinfuser, can even benefit not only developers, but also UX designers who prototype}




\subsection{Improving User Experience, Trust, and Adoption}\label{sec:importance-ux}

When developing user experiences powered by LLMs, respondents emphasized the importance of being able to constrain LLMs and mitigate hallucinations to enhance user experience, foster trust, and drive customer adoption (\temp{xx\%}). One prominent aspect is to eliminate safety and privacy concerns, for example, \userquote{it would be nice to know that the summarization will not repeat existing PII (personally identifiable information) or hallucinate some PII from the prompt.} In addition, respondents expressed a desire to ensure user trust and confidence of LLM-powered tools and systems, arguing that, for instance, \userquote{hallucinations in dates are easy to identify by the user} and \userquote{users won't invest more time into tools that aren't accurate.} Relatedly, one respondent who self-identified as a product manager wished that \userquote{it will greatly help to be accurate in all customer demos I make} in order to increase user adoption of their product.

% \userquote{replacing all occurrences of [personally identifiable information] with innocuous placeholders.}



% \temp{
% Improve user trust and confidence
% Increase customer satisfaction and adoption
% Eliminate privacy / safety concerns
% }

==> sections/old_sections/sec-033-gui-nl-20240105.tex <==
\section{Case Study: How to Specify Constraints}\label{sec:gui-or-nl}



\begin{table*}[t]
\centering
\vspace{-2mm}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{
p{27mm}|
p{24mm}|
p{24mm}|
p{28mm}|
p{24mm}|
p{33mm}|
p{27mm}
}
\toprule
~ &
Output should be exactly 3 words, no more than 3 paragraphs, etc. &
Only output ``left-handed'', ``right-handed'', or ``ambidextrous'' &
Output in a specific format or structure (e.g., JSON, XML, bulleted / ordered list) &
Output must include or avoid certain words / phrases &
Output must cover or avoid certain topics, only use certain libraries when generating code, etc. &
Output should mimic Yoda / Shakespeare / certain personas, etc.) \\\midrule

\textbf{Mean score (stdev)} & 
4.22 ($\pm$ 1.91) &
4.04 ($\pm$ 1.95) &
4.24 ($\pm$ 2.11) &
3.70 ($\pm$ 2.00) &
3.44 ($\pm$ 1.83) & 
3.04 ($\pm$ 1.71) \\\midrule

\textbf{\# of participants who preferred\newline NL / Neutral / GUI} &
14 / 13 / \textbf{23} &
17 / 12 / \textbf{21} &
15 / 10 / \textbf{25} &
\textbf{20} / 13 / 17 &
\textbf{23} / 15 / 12 &
\textbf{31} / 12 / 7 \\\bottomrule
\end{tabular}
}
\caption{Respondents' preferences towards specifying output constraints either through natural language or GUI. Participants were asked to provide a score for question (column) on a 7-point Likert scale from 1 (strongly prefer natural language (NL)) to 7 (strongly prefer GUI). 
For the last row, we place participants
who preferred NL (score < 4), neutral (score = 4), or GUI (score > 4) into their respective buckets and report the bucket sizes (with the largest bucket bolded).}
\label{tab:gui-nl-table}
\vspace{-3mm}
\end{table*}


Recall that, as a case study that probes participants' thoughts on diverse ways of conveying output constraints to an LLM beyond simply using natural language prompts, we introduced the concept of using a graphical user interface (GUI) as a viable alternative.
As a result, table \ref{tab:gui-nl-table} shows respondents' preferences towards specifying output constraints either through GUI or natural language. An overarching observation is that respondents preferred using GUI to specify low-level constraints (e.g., length, formatting, structured output) and natural language to express high-level constraints (semantic, stylistic, etc.). In addition, respondents also expressed detailed rationale of their preferences through open text responses:


\subsection{The case for GUI: Quick, Flexible, and Ease of Mind}

First and foremost, respondents considered GUI particularly useful for defining \userquote{hard requirements [...] that need to be definitely followed.} In these scenarios, they suggested that GUI can offer a greater perceived assurance of expected outcomes, due to the reduced ambiguity and increased consistency compared to using natural language --- for example, one respondent felt that \userquote{if I type that I want a Yes / No response and write it in a prompt, the request may not be honoured. I perceive that requests made in GUI controls will be honoured,} while another claimed that \userquote{flagging a `JSON' button} provides a much better user experience than \userquote{typing `output as JSON' across multiple prompts.}
In addition, respondents preferred using GUI when the intended constraint is \userquote{objective},  \userquote{quantifiable} or only involves a finite set of variants or options, such as \userquote{number of words in the response}, \userquote{use only items x,y,z,} or \userquote{a JSON with certain fields specified.}
Moreover, respondents regarded GUI as more flexible and suitable for rapidly prototyping and experimenting with constraints independent of the prompt (e.g., \userquote{when I want to play around with different numbers, moving a slider around seems easier than typing something}), which can be particularly beneficial during user testing (e.g., \userquote{testing different modes of interaction and controls with users is easier by quickly toggling [UI knobs]}).
Last but not least, for less experienced LLM users, the range of choices for a constraint afforded by a GUI can help improve their understanding of model capabilities and limitations, making the model seems less like a black box. One respondent drew from their experience working with text-to-image models to underscore this point: \userquote{by seeing ``Illustration'' as an output style [among others like ``Photo realistic'' or ``Cartoon''], I became aware of [the model's] capabilities.}



\subsection{The Case for NL: More Intuitive and Expressive for Complex Constraints}
Compared to using GUI, respondents found it easier and more flexible to describe the intended constraint using natural language when it involves an extended context or a large number of choices that couldn't reasonably fit into a GUI. For example, one respondent noted the ease of providing background information to LLMs using natural language, such as specifying \userquote{these are meetings, these are emails, etc...} 
In addition, respondents preferred natural language over GUI when the constraint itself is \userquote{vague}, \userquote{nuanced} or \userquote{open-ended}, such as \userquote{don't include offensive words} or \userquote{respond in a cheerful manner.} Furthermore, some emphasized that natural language provides a more natural, familiar, and expressive way to communicate (potentially multiple) complex constraints to the model, and in these situations, they imagine that \userquote{trying to figure out how to use a GUI might be more tedious than just writing it out.}




% However, as discussed in \temp{section x (forward ref)}, constraints described in natural language can be inherently ambiguous and ...

% such as \userquote{[when] I need to give the LLM some context (e.g., these are meetings, these are emails, etc...)} or \userquote{controlling the length of output, such as the number of words, characters, tokens, sentences, paragraphs, conjunctions, clauses, etc.}




\subsection{Additional Needs}

Respondents conceded that, despite their oftentimes preference for GUI support when defining constraints, they ultimately need to translate everything into natural language within the prompt, as this is the only way to add constraints given the current state of API support. In addition, some expressed a desire to \userquote{link to external resources} when describing constraints (e.g., \userquote{a large database / vocabulary}) that would be impractical to \userquote{inputted directly as a prompt} through the current APIs.  This implies that it could be advantageous to provide a separate ``post-prompt'' API field exclusively for developers to detail output constraints, potentially through the use of a formal language or notation.\looseness=-1



% \temp{
% API support

% link to external resources

% creative use cases - give more weight to unique instructions in the prompt

% Providing learning opportunity for when/where to apply what constraints (on-ramp for NL constraints)
% }

==> sections/old_sections/sec-040-tool-2024-0105.tex <==
\section{The \systemname Tool}

\begin{figure*}[t]
\centering
\vspace{-4mm}
\includegraphics[width=1.0\linewidth]{assets/images/tool-crop.pdf}
\vspace{-7mm}
\caption{\systemname's user interfaces (1-4) \& use cases (5-6). After writing the prompt (1), users can easily specify output constraints using a graphical user interface (2 \& 3) provided by \systemname, and the resulting output (4) is guaranteed to follow the constraints. Additional details of this process is discussed in section \ref{sec:tool-ui}.}
\label{fig:tool}
\vspace{-3mm}
\end{figure*}




Informed by the results of the survey, we developed a web-based tool, \systemname (Figure \ref{fig:tool}), that enables LLM users to prototype, test, and apply constraints on the \emph{format} of LLM outputs. \temp{\systemname also incorporates a version of the LLM detailed in \cite{team_gemini_2023}, which is a specialized LLM that is promptable in the same way as \gptFour \cite{openai_gpt-4_2023} and can simultaneously accept a piece of constraint specified using a DSL (details below).} We first delve into the workflow of using \systemname, followed by a discussion of our initial observations gathered from the preliminary user tests of the tool.\looseness=-1


\subsection{Creating Constraints}\label{sec:tool-ui}
To illustrate the process of creating an output constraint, consider an example prompt of ``Generate a character profile for a video game, including the character's name, age, names of their three children, and whether they can be controlled by the player'' (Figure \ref{fig:tool}-1), and instead of letting the LLM decide the format of the output, the user would like to constrain the output to be a custom JSON object. 
To achieve this, they can simply click the ``JSON object'' button among the list of available constraint \emph{primitives} (Figure \ref{fig:tool}-2b) to place it onto the constraint \emph{line} (Figure \ref{fig:tool}-2a). 
To further edit the schema of the JSON object, the user can hover over the JSON object primitive and click the edit button (pencil icon) to bring up the editing popup modal (Figure \ref{fig:tool}-3). There, they can input the desired keys of the expected fields, in this case, \texttt{name}, \texttt{age}, \texttt{children} and \texttt{playable}. The default data type of each field is a JavaScript \texttt{string}, but the user can further tweak it to be either a \texttt{number}, an \texttt{array}, and \texttt{a boolean} (Figure \ref{fig:tool}-3a). 
% After clicking on the ``Save'' button, the fine-grained edits will be reflected on the original JSON object primitive.

Note that users have the flexibility to mix and match multiple constraint primitives together as well as edit (if applicable) and remove any primitives. 
For instance, Figure \ref{fig:tool}-6 shows a constraint that consists of two primitives, an ``Exact text'' primitive with the value ``\texttt{Sentiment :}'' and a ``Multiple choice'' primitive with the available choices being \texttt{positive}, \texttt{negative}, or \texttt{neutral}. 
Currently, based on the needs and priorities identified by the survey, \systemname supports ``JSON object,'' ``Multiple choice,'' ``List,'' ``Ordered list,'' ``Some text,'' and ``Exact text,'' where ``Some text'' asks the LLM to generate freely as it normally would, and ``Exact text'' asks the LLM to insert the exact text that users specified during generation.\looseness=-1

In addition, \systemname automatically translates the constraint specified using the GUI into a regular expression-based domain specific language (hereafter referred to as ``regex'') that our specialized backend LLM can recognize and follow (Figure \ref{fig:tool}-2d). \temp{should probably go into a little bit more detail on how this works, citing \cite{willard_efficient_2023}.} 
This regex is by default read-only and can be toggled as hidden through the ``< >'' button (Figure \ref{fig:tool}-2c), however, for more advanced users, they can toggle on the ``Edit constraints manually'' button to directly manipulate the regex based on their specific needs.
Ultimately, the output will strictly adhere to the given constraint, namely, a JSON object with the specified fields (Figure \ref{fig:tool}-4). this is in contrast to the output from a standard LLM without this constraint --- according to our findings, users cannot ensure receiving a valid and parsable JSON object, nor can they anticipate a consistent schema within the JSON.


% \temp{available regex primitives, how it works, maybe in appendix?}



\subsection{Initial Observations}
To explore the usability and usefulness of \systemname, we conducted a series of 6 informal user tests with both some of the authors themselves and additional participants who self-identified as experts in prompting LLMs. Sessions lasted between 30 minutes and one hour and were conducted via an online video conferencing tool. We describe the initial findings below, but leave rigorous evaluation and analysis of a more full-fledged \systemname to future work.

Contrary to the traditional approach in LLM prompting, where users must articulate constraints using natural language within the prompt, \systemname allows users to separate ``the tasks they want the model to perform'' from ``the expected format of the output.'' Participants generally found this separation of concern more intuitive and effective in steering LLMs to consistently achieve desired results. 
Additionally, although prompts and constraints still have a one-to-one mapping in \systemname, some participants envisioned the potential for sharing and reusing constraints across different prompts. This could both offset the initial effort required to craft an effective constraint for a series of similar prompts, and eliminate the need for traditional prompt engineering following model migration.

One particularly intriguing opportunity as well as feature request involves enabling \systemname to automatically deduce the suitable constraint based on the user-written prompt. For instance, after users write the prompt as shown in Figure \ref{fig:tool}-1, \systemname could automatically suggest corresponding constraints. The system might proactively ask users if they'd like to restrain the model output to a JSON object with relevant fields. 
This feature is appealing considering the currently tedious nature of manually crafting and modifying constraint primitives from scratch. Inspired by code auto-completion, participants suggested that constraint auto-completion could enhance the overall experience of defining constraints, making it quicker and more seamless.
Furthermore, for those new to using \systemname, these automatically suggested constraints could serve as valuable learning tools. They can assist users in familiarizing themselves with the tool, especially in future versions where the tool might support an expanded array of constraint primitives.
Last but not least, proactively suggesting constraints could help foster a ``constraint mindset'' --- it could remind users to always reason able the format of the output before deploying a prompt, ultimately making prompt engineering and development more rigorous and controllable, akin to traditional software engineering.



% However, current process of coming up with an effective constraint for a prompt can still be haphazard. Participants found that they often have to tweak the constraint and the prompt simultaneously to have them ``sync up'' 
% orchestration

% can we achieve a true separation of concern needs additional future research.

% \temp{match constraint with prompt, but could have limited generalizability}




% \subsubsection{Proactively helping users author constraints}

% \temp{things get long, then might forget}


% \temp{infer constraints from prompt}






==> sections/old_sections/sec-050-discussion.tex <==
\section{Discussion}

\temp{
- Users' needs might be themselves constrained by the perceived capabilities of the model, when model capabilities improve, new user needs might emerge
}

\temp{how to address the constraints, either through constrained decoding or SFT}

\temp{more customization of LLMs, lack of ``fine-grained control knobs''}
